Learning to Represent Edits

We introduce the problem of learning distributed representations of edits. By combining a "neural editor" with an "edit encoder", our models learn to represent the salient information of an edit and can be used to apply edits to new inputs. We experiment on natural language and source code edit data. Our evaluation yields promising results that suggest that our neural network models learn to capture the structure and semantics of edits. We hope that this interesting task and data source will inspire other researchers to work further on this problem.

==> Makefile <==

all:
	latexmk -pdf -bibtex editrepresentations.tex

clean:
	latexmk -C

spell:
	find ./ -type f -name "*.tex" -exec aspell --per-conf=./etc/aspell.cfg/aspell.conf -p ./etc/aspell.cfg/aspell.en.pws -c "{}" \;


==> text/codesamples.tex <==
% \label{app:codesamples}
% \begin{table}[h]
% \resizebox{\columnwidth}{!}{
    
% \footnotesize
% \begin{tabular}{ll} \toprule
%  &\elementbefore: \lstinline|V0.TryGet(nameof(V1), out long etag);| \\
%      &\elementafter: \lstinline|V0.TryGet(nameof(V1), out long? etag);|\\ \midrule

% \multicolumn{2}{l}{\underline{Bag of Words}} \\
% $\blacktriangleright$ & \elementbefore: \lstinline|V0= LIT + V1.Author ?? LIT;|\\
%                       & \elementafter: \lstinline|V0= LIT + (V1.Author ?? LIT);|\\ \rowspace
% $\blacktriangleright$ & \elementbefore: \lstinline|string V0= GetComment(V1);|\\
%                       & \elementafter: \lstinline|string[] V0= GetComment(V1);|\\
% \midrule

% \multicolumn{2}{l}{\underline{Seq2Seq -- Seq Edit Encoder}} \\
% $\blacktriangleright$ & \elementbefore: \lstinline|var V0= new LibraryManager(V1.Values.ToList(), V2, V3.ProjectFilePath);|\\
%                       & \elementafter: \lstinline|var V0= new LibraryManager(V1.Values.ToList(), V2, V3?.ProjectFilePath);|\\ \rowspace
% $\blacktriangleright$ & \elementbefore: \lstinline|Format(V0.GetElementType(), V1= V2.Dereference());|\\
%                       & \elementafter: \lstinline|Format(V0.GetElementType(), V1= V2?.Dereference());|\\
% \midrule


% \multicolumn{2}{l}{\underline{Graph2Tree -- Seq Edit Encoder}} \\
% $\blacktriangleright$ & \elementbefore: \lstinline|_ilg.EmitConvertToType(TypeUtils.GetNonNullableType(V0), V0, true);|\\
%                       & \elementafter: \lstinline|_ilg.EmitConvertToType(TypeUtils.GetNonNullableType(V0), V0, isChecked: true);|\\ \rowspace
% $\blacktriangleright$ & \elementbefore: \lstinline|_ilg.EmitConvertToType(V0, typeof(int), true);|\\
%                       & \elementafter: \lstinline|_ilg.EmitConvertToType(V0, typeof(int), isChecked: true);|\\
% \midrule

% \multicolumn{2}{l}{\underline{Graph2Tree -- Graph Edit Encoder}} \\
% $\blacktriangleright$ & \elementbefore: \lstinline|V0.Verify(V1=>V1.Challenge(new string[]\{\}, null));|\\
%                       & \elementafter: \lstinline|V0.Verify(V1=>V1.Challenge(null, (IEnumerable<string>)new string[]\{\}));|\\ \rowspace
% $\blacktriangleright$ & \elementbefore: \lstinline|Assert.Equal((short)(V0/ V1), V2());|\\
%                       & \elementafter: \lstinline|Assert.Equal((short?)(V0/ V1), V2());|\\
%     \bottomrule
% \end{tabular}
% } % resizebox
% \end{table}


% \begin{table}[h]
%     \resizebox{\columnwidth}{!}{
        
%     \footnotesize
%     \begin{tabular}{ll} \toprule
%      &\elementbefore: \lstinline|V0= V1.ToHeaders().ToNameValueCollection();| \\
%          &\elementafter: \lstinline|V0= new NameValueCollectionWrapper(V1.ToHeaders().ToNameValueCollection());|\\ \midrule
    
%     \multicolumn{2}{l}{\underline{Bag of Words}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|var V0= new NameValueCollection();|\\
%                           & \elementafter: \lstinline|var V0= NameValueCollectionWrapper.New();|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|this.V0= new NameValueCollection();|\\
%                           & \elementafter: \lstinline|var V0= NameValueCollectionWrapper.New();|\\
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Seq2Seq -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= V1.CreateNewWriter();|\\
%                           & \elementafter: \lstinline|V0= new DataFormatter(V1.CreateNewWriter());|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= Language.CamelCase(V1);|\\
%                           & \elementafter: \lstinline|V0= new DescribeAttribute(Language.CamelCase(V1));|\\
%     \midrule
    
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= V1.CreateNewWriter();|\\
%                           & \elementafter: \lstinline|V0= new DataFormatter(V1.CreateNewWriter());|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= Language.CamelCase(V1);|\\
%                           & \elementafter: \lstinline|V0= new DescribeAttribute(Language.CamelCase(V1));|\\
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Graph Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= V1.CreateNewWriter();|\\
%                           & \elementafter: \lstinline|V0= new DataFormatter(V1.CreateNewWriter());|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= Language.CamelCase(V1);|\\
%                           & \elementafter: \lstinline|V0= new DescribeAttribute(Language.CamelCase(V1));|\\
%         \bottomrule
%     \end{tabular}
%     } % resizebox
% \end{table}

% \begin{table}[h]
%     \resizebox{\columnwidth}{!}{
        
%     \footnotesize
%     \begin{tabular}{ll} \toprule
%      &\elementbefore: \lstinline|this.V0= new SuperSimpleViewEngine();| \\
%          &\elementafter: \lstinline|this.V0= new SuperSimpleViewEngine(new FakeViewEngineHost());|\\ \midrule
    
%     \multicolumn{2}{l}{\underline{Bag of Words}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|await TestAsync(LIT, LIT, options: UseImplicitTypeTests.ImplicitTypeEverywhere());|\\
%                           & \elementafter: \lstinline|await TestAsync(LIT, LIT, options: new UseImplicitTypeTests().ImplicitTypeEverywhere());|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|await TestAsync(LIT, LIT, options: UseImplicitTypeTests.ImplicitTypeButKeepIntrinsics());|\\
%                           & \elementafter: \lstinline|await TestAsync(LIT, LIT, options: new UseImplicitTypeTests().ImplicitTypeButKeepIntrinsics());|\\
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Seq2Seq -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|this.V0= new NancyOptions();|\\
%                           & \elementafter: \lstinline|this.V0= new NancyOptions(new DefaultNancyBootstrapper());|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= new GKMatchmakerViewController();|\\
%                           & \elementafter: \lstinline|V0= new GKMatchmakerViewController(new GKMatchRequest());|\\
%     \midrule
    
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|this.V0= new NancyOptions();|\\
%                           & \elementafter: \lstinline|this.V0= new NancyOptions(new DefaultNancyBootstrapper());|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= new GKMatchmakerViewController();|\\
%                           & \elementafter: \lstinline|V0= new GKMatchmakerViewController(new GKMatchRequest());|\\
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Graph Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= new GKMatchmakerViewController();|\\
%                           & \elementafter: \lstinline|V0= new GKMatchmakerViewController(new GKMatchRequest());|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= new HashSet<PropertyKey>();|\\
%                           & \elementafter: \lstinline|V0= new HashSet<PropertyKey>(new PropertyKeyEqualityComparer());|\\
%         \bottomrule
%     \end{tabular}
%     } % resizebox
% \end{table}

% \begin{table}[h]
%     \resizebox{\columnwidth}{!}{
        
%     \footnotesize
%     \begin{tabular}{ll} \toprule
%      &\elementbefore: \lstinline|V0= V1.Create(nameof(SolutionAttributes), this);| \\
%          &\elementafter: \lstinline|V0= V1.Create(this, nameof(SolutionAttributes));|\\ \midrule
    
%     \multicolumn{2}{l}{\underline{Bag of Words}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.Add(V1, new EnumMember(V1, this, V2, V3));|\\
%                           & \elementafter: \lstinline|V0.Add(V1, new EnumMember(this, V1, V2, V3));|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= V1.Create(nameof(ProjectAttributes), this);|\\
%                           & \elementafter: \lstinline|V0= V1.Create(this, nameof(ProjectAttributes));|\\
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Seq2Seq -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= V1.Create(nameof(ProjectAttributes), this);|\\
%                           & \elementafter: \lstinline|V0= V1.Create(this, nameof(ProjectAttributes));|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= V1.Create(nameof(DocumentAttributes), this);|\\
%                           & \elementafter: \lstinline|V0= V1.Create(this, nameof(DocumentAttributes));|\\
%     \midrule
    
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= V1.Create(nameof(DocumentAttributes), this);|\\
%                           & \elementafter: \lstinline|V0= V1.Create(this, nameof(DocumentAttributes));|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= V1.Create(nameof(ProjectAttributes), this);|\\
%                           & \elementafter: \lstinline|V0= V1.Create(this, nameof(ProjectAttributes));|\\
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Graph Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= V1.Create(nameof(ProjectAttributes), this);|\\
%                           & \elementafter: \lstinline|V0= V1.Create(this, nameof(ProjectAttributes));|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= V1.Create(nameof(DocumentAttributes), this);|\\
%                           & \elementafter: \lstinline|V0= V1.Create(this, nameof(DocumentAttributes));|\\
%         \bottomrule
%     \end{tabular}
%     } % resizebox
% \end{table}

% \begin{table}[h]
%     \resizebox{\columnwidth}{!}{
        
%     \footnotesize
%     \begin{tabular}{ll} \toprule
%      &\elementbefore: \lstinline|V0.Add(new Customer().Parse(V1));| \\
%          &\elementafter: \lstinline|V0.Add(Parse(V1));|\\ \midrule
    
%     \multicolumn{2}{l}{\underline{Bag of Words}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.Subscribe(Self, new[] \{ typeof(ClusterEvent.IMemberEvent) \});|\\
%                           & \elementafter: \lstinline|V0.Subscribe(Self, typeof(ClusterEvent.IMemberEvent));|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|var V0= V1.MakeGenericMethod(new[] { V2});|\\
%                           & \elementafter: \lstinline|var V0= V1.MakeGenericMethod(V2);|\\
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Seq2Seq -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.Add(new Country().Parse(V1));|\\
%                           & \elementafter: \lstinline|V0.Add(Parse(V1));|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.Add(new City().Parse(V1));|\\
%                           & \elementafter: \lstinline|V0.Add(Parse(V1));|\\
%     \midrule
    
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.Add(new City().Parse(V1));|\\
%                           & \elementafter: \lstinline|V0.Add(Parse(V1));|\\\rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.Add(new Address().Parse(V1));|\\
%                           & \elementafter: \lstinline|V0.Add(Parse(V1));|\\
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Graph Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.Add(new Address().Parse(V1));|\\
%                           & \elementafter: \lstinline|V0.Add(Parse(V1));|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.Add(new City().Parse(V1));|\\
%                           & \elementafter: \lstinline|V0.Add(Parse(V1));|\\
%         \bottomrule
%     \end{tabular}
%     } % resizebox
% \end{table}

% \begin{table}[h]
%     \resizebox{\columnwidth}{!}{
        
%     \footnotesize
%     \begin{tabular}{ll} \toprule
%      &\elementbefore: \lstinline|V0=PageValueFor(V1.Base+V1.FixedSize_StartPosition, V1.LastSearchPosition);| \\
%          &\elementafter: \lstinline|V0=PageValueFor(V1.Base+V1.FixedSize_StartPosition, 0);|\\ \midrule
    
%     \multicolumn{2}{l}{\underline{Bag of Words}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|var V0= GetSeparatorKeyAtPosition(V1, V2.LastSearchPosition);|\\
%                           & \elementafter: \lstinline|var V0= GetSeparatorKeyAtPosition(V1, 0);|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= V1.AddNode(V1.LastSearchPosition, V2, V3, V4);|\\
%                           & \elementafter: \lstinline|V0= V1.AddNode(V5, V2, V3, V4);|\\
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Seq2Seq -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|System.Threading.LockCookie V0= V1.UpgradeToWriterLock(int.MaxValue);|\\
%                           & \elementafter: \lstinline|System.Threading.LockCookie V0= V1.UpgradeToWriterLock(0);|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|ConsumeLayout((int)(V0- V1), (int)V2);|\\
%                           & \elementafter: \lstinline|ConsumeLayout((int)(V0- V1), 0);|\\
%     \midrule
    
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|var V0= GetSeparatorKeyAtPosition(V1, V2.LastSearchPosition);|\\
%                           & \elementafter: \lstinline|var V0= GetSeparatorKeyAtPosition(V1, 0);|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline{V0|= ConsumeLayout((int)(V1- V2), (int)V3);}\\
%                           & \elementafter: \lstinline{V0|= ConsumeLayout((int)(V1- V2), 0);}\\
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Graph Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline{V0|= ConsumeLayout((int)(V1- V2), (int)V3);}\\
%                           & \elementafter: \lstinline{V0|= ConsumeLayout((int)(V1- V2), 0);}\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|this.AddActionWidget(this.V0, -LIT);|\\
%                           & \elementafter: \lstinline|this.AddActionWidget(this.V0, 0);|\\
%         \bottomrule
%     \end{tabular}
%     } % resizebox
% \end{table}


% \begin{table}[h]
%     \resizebox{\columnwidth}{!}{
        
%     \footnotesize
%     \begin{tabular}{ll} \toprule
%      &\elementbefore: \lstinline|V0.RecordTransformationError(V1);| \\
%          &\elementafter: \lstinline|V0.RecordTransformationError(V1, V2.DocumentId);|\\ \midrule
    
%     \multicolumn{2}{l}{\underline{Bag of Words}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.WriteJson(new \{ Error = LIT + V1+ LIT \});|\\
%                           & \elementafter: \lstinline|V0.WriteJson(new \{ Error = LIT + V2.DocumentId + LIT \});|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|var V0= V1.Search(new TermQuery(new Term(Constants.DocumentIdFieldName, V2)), 1);|\\
%                           & \elementafter: \lstinline|var V0= V1.Search(new TermQuery(new Term(Constants.DocumentIdFieldName, V3.DocumentId)), 1);|\\
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Seq2Seq -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.m_componentBlocks.Add(V1);|\\
%                           & \elementafter: \lstinline|V0.m_componentBlocks.Add(V1, V2.Main);|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0?.Invoke(V1);|\\
%                           & \elementafter: \lstinline|V0?.Invoke(V1, V2.Flags);|\\
%     \midrule
    
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.m_componentBlocks.Add(V1);|\\
%                           & \elementafter: \lstinline|V0.m_componentBlocks.Add(V1, V2.Main);|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.Indexing.AddIndex(V1);|\\
%                           & \elementafter: \lstinline|V0.Indexing.AddIndex(V1, V2.IsMapReduce);|\\
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Graph Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.Apply(V1);|\\
%                           & \elementafter: \lstinline|V0.Apply(V1, V2.Object);|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0.Emit(V1);|\\
%                           & \elementafter: \lstinline|V0.Emit(V1, V2.CodeGen);|\\
%         \bottomrule
%     \end{tabular}
%     } % resizebox
% \end{table}


% \begin{table}[h]
%     \resizebox{\columnwidth}{!}{
        
%     \footnotesize
%     \begin{tabular}{ll} \toprule
%      &\elementbefore: \lstinline|bool V0= true;| \\
%          &\elementafter: \lstinline|bool V0= CanBeNull(V1);|\\ \midrule
    
%     \multicolumn{2}{l}{\underline{Bag of Words}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= true;|\\
%                           & \elementafter: \lstinline|V0= !V1;|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|V0= true;|\\
%                           & \elementafter: \lstinline|V0= !V1;|\\ 
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Seq2Seq -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|string V0= LIT;|\\
%                           & \elementafter: \lstinline|string V0= InvariantToString(V1);|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|string V0= LIT;|\\
%                           & \elementafter: \lstinline|string V0= InvariantToString(V1);|\\ \\
%     \midrule
    
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Seq Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|int V0= 0;|\\
%                           & \elementafter: \lstinline|int V0= SkipViewstate(V1);|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|string V0= LIT;|\\
%                           & \elementafter: \lstinline|string V0= InvariantToString(V1);|\\
%     \midrule
    
%     \multicolumn{2}{l}{\underline{Graph2Tree -- Graph Edit Encoder}} \\
%     $\blacktriangleright$ & \elementbefore: \lstinline|string V0= LIT;|\\
%                           & \elementafter: \lstinline|string V0= InvariantToString(V1);|\\ \rowspace
%     $\blacktriangleright$ & \elementbefore: \lstinline|string V0= LIT;|\\
%                           & \elementafter: \lstinline|string V0= InvariantToString(V1);|\\ 
%         \bottomrule
%     \end{tabular}
%     } % resizebox
% \end{table}

==> text/nlsamples.tex <==
\begin{table}[h]
\footnotesize
\begin{tabular}{lp{6cm}p{6cm}} \toprule
    \multicolumn{3}{p{\columnwidth}}{may was educated at \insertText{sydney boys high school and then} the university of sydney , reading chemical engineering and theoretical physics ( bsc 1956 ) and receiving a phd in theoretical physics in 1959 .}\\
    NN-1 & it was founded in 1924 \insertText{as boys high school} , and renovated once in 1950 , once in 1987 , and once again in 2004 . & after attending school at \insertText{rondebosch boys ' high school and then} western province preparatory school and diocesan college , shuttleworth obtained a business science degree in finance and information systems at the university of cape town .\\
    NN-2 & mcdonald was born in drummoyne , new south wales , australia , in 1935 \insertText{and was educated at drummoyne boys high school and sydney technical high school .} & holding degrees from \insertText{alief elsik high school ,} the university of houston , eastman school of music , and yale university , he has been a hailed as one of the leading composers of his generation .\\
    NN-3 & kutama college , formed before 1940 , is the commonly used name for st. francis xavier 's college \insertText{, an all - boys high school} in the rural area of zvimba in zimbabwe , about 80 kilometres southwest of the capital harare . & shawcross was educated at \insertText{st. aubyns preparatory school , rottingdean ,} eton college and university college , oxford , and worked as a journalist for '' the sunday times '' .\\
    \bottomrule
\end{tabular}   
\end{table}

\begin{table}[h]
\footnotesize
\begin{tabular}{lp{6cm}p{6cm}} \toprule    
    \multicolumn{3}{p{15cm}}{Initial}\\ \midrule
        & Bag of Words & Seq2Seq -- Seq Edit Encoder \\ \midrule
    NN-1 & S1 & S1\\
    NN-2 & S2 & S2\\
    NN-3 & S3 & S3\\
    \bottomrule
\end{tabular}   
\end{table}

\begin{table}[h]
\footnotesize
\begin{tabular}{lp{6cm}p{6cm}} \toprule    
    \multicolumn{3}{p{15cm}}{Initial}\\ \midrule
        & Bag of Words & Seq2Seq -- Seq Edit Encoder \\ \midrule
    NN-1 & S1 & S1\\
    NN-2 & S2 & S2\\
    NN-3 & S3 & S3\\
    \bottomrule
\end{tabular}   
\end{table}

\begin{table}[h]
\footnotesize
\begin{tabular}{lp{6cm}p{6cm}} \toprule    
    \multicolumn{3}{p{15cm}}{Initial}\\ \midrule
        & Bag of Words & Seq2Seq -- Seq Edit Encoder \\ \midrule
    NN-1 & S1 & S1\\
    NN-2 & S2 & S2\\
    NN-3 & S3 & S3\\
    \bottomrule
\end{tabular}   
\end{table}
